A Deep Dive into the Disparity of Word Error Rates Across Thousands of NPTEL MOOC Videos

Automatic speech recognition (ASR) systems are designed to transcribe spoken language into written text and find utility in a variety of applications including voice assistants and transcription services. However, it has been observed that state-of-the-art ASR systems which deliver impressive benchmark results, struggle with speakers of certain regions or demographics due to variation in their speech properties. In this work, we describe the curation of a massive speech dataset of 8740 hours consisting of $\sim9.8$K technical lectures in the English language along with their transcripts delivered by instructors representing various parts of Indian demography. The dataset is sourced from the very popular NPTEL MOOC platform. We use the curated dataset to measure the existing disparity in YouTube Automatic Captions and OpenAI Whisper model performance across the diverse demographic traits of speakers in India. While there exists disparity due to gender, native region, age and speech rate of speakers, disparity based on caste is non-existent. We also observe statistically significant disparity across the disciplines of the lectures. These results indicate the need of more inclusive and robust ASR systems and more representational datasets for disparity evaluation in them.

==> Evaluation.tex <==
\section{Evaluation Dataset and Methodology}
In the upcoming sections, we will discuss the process used for the dataset selection, collection and annotation for associated metadata and the how have used the prepared dataset for examining bias in YouTube Captions and OpenAI Whisper.

\subsection{Dataset Curation}

 Our objective is to create a large corpus of Indian speakers English speech dataset along with the associated ground truth transcripts which is not only acoustically varied but also linguistically rich to satisfactorily answer our research questions.The speech dataset needs to have labels corresponding to speaker social traits like gender, age, caste, native region etc and also labels categorizing speech content in different categories.

\subsubsection{Dataset Collection}
Keeping the view the properties of dataset required for our work, we have preferred recorded technical monologues delivered by Indian university lecturers. The monologues audio are generally less noisy than lectures delivered in interactive settings and it help us in avoiding the speech pre-processing and enhancement tasks which could potentially add bias in our dataset.

Some of the examples of publicly avaliable pre-recorded university lectures dataset are following:
\begin{itemize}
    \item The National Programme on Technology Enhanced Learning (NPTEL) is an initiative in India that provides free online courses and video lectures in engineering and other technical disciplines. The NPTEL video lectures are available on YouTube and many of them have transcripts available in English and other Indian languages
    \item The MIT OpenCourseWare (OCW) is a free and open digital publication of MIT course materials that includes video lectures, transcripts, and other educational resources with focus primarily on technical subjects
    \item The Open Learning Initiative (OLI) at Carnegie Mellon University is another resource that provides free online courses and video lectures in a variety of technical subjects.These lectures are mainly focussed around topics from computer science and engineering and have transcripts data available too.
    \item The Coursera platform is a commercial provider of online courses, including many technical courses lectures along with their transcripts
\end{itemize}

We have chosen the NPTEL YouTube hosted engineering domain lectures as the source of our dataset as our focus is on ASR performance in Indian context and also due to the convenience and accessibility of the lectures along with their manual and YouTube Captions generated transcripts.We have only selected those YouTube video lectures for which both manual and YouTube Captions generated English transcripts are available.

\subsubsection{Dataset Labelling}
To complete our curation step, we add, for each lecture, labels representing individual characteristics of each instructor like gender, caste, age group, native accent and the labels representing the lecture content category.

For accomplishing our labelling task we first scrapped the NPTEL website for the metadata readily present for each lecture. The information corresponding to each lecture we got from the NPTEL website are Course Name, Discipline Name, Institution Name, Instructor Name and YouTube URL.

As the metadata does not contain any demographic related information of the lecturer, we need to devise a method that reliably derives it.For gender and caste category labelling of instructors, their full names are used to run inference on pre-trained model proposed by ~\cite{https://doi.org/10.48550/arxiv.2209.03089}.The Indian names vary significantly not only for individual's gender but also for individual's caste, religion and native state. The same has been leveraged by the model 
 ~\cite{https://doi.org/10.48550/arxiv.2209.03089} which has been trained on large labelled corpus of Indian names. 
 
 Note that our definition of gender represents the perceived gender, and not necessarily the self-identified gender of the instructor. Similarly, the caste of individual speakers represents the perceived caste category which depends mostly on the last names of individuals. As per many existing castes prevalent in Indian demography \footnote{$https://en.wikipedia.org/wiki/Caste_system_in_India$} , we have categorized the castes into two broad groups, reserved (SC/ST/OBC) and unreserved caste groups based on existing reservation system \footnote{$https://en.wikipedia.org/wiki/Reservation_in_India$} in India.

We were unable to find out any programmatic way to label the age group of instructors as the date or even year of birth of most instructors is  not available in public domain. So we have tried to estimate their approximate age group using the information about they have started their academic career. We were able to find the year year in which each lecturer started their career from their their curriculum vitae (CV) or profile page available on their currently associated institute website. We have created four seniority categories for lecturers who began their careers before 1980 , between 1980- 1990 , between 1990 - 2000 and after 2000 and marked them as Very Senior, Senior, Junior and Very Junior respectively.  

 We annotated the non-demographic label, speech rate which is derived  by dividing the total number of words in the ground-truth transcript by the lecture duration.Speech rate is a measure of word utterance rate of the instructor and calculated in terms of words per minute(wpm).

Finally we grouped the discipline name metadata of each lecture into two groups engineering and non-engineering. We have marked those disciplines as engineering which traditionally involves the application of physical and mathematical principles to solve real-world problems like Aerospace Engineering, Civil Engineering, Mechanical Engineering etc while those disciplines like Mathematics , Management , Humanities etc in which abstract concepts , ideas and theories are of primary focus are marked as non-engineering disciplines. The detailed list of disciplines in both categories can be found in Appendix 1. Please note that this classification is based on the traditional definitions of engineering and non-engineering disciplines, and there may be some overlap between the two categories. For example, computer science and engineering is typically considered an engineering discipline, but it may also involve elements of mathematics and computer science, which are typically considered non-engineering disciplines. Similarly, agriculture may involve elements of biology, chemistry, and other scientific disciplines, but it is typically considered a non-engineering discipline.












\subsubsection{Transcripts Generation}
After having collected all metadata corresponding to each lecture and labelling the demographic characteristics of the speaker , we obtained the ground truth transcripts and YouTube Captions generated transcripts using the Python YoutubeTranscript API ~\cite{pypiYoutubetranscriptapi}. The textual part of the transcripts corresponding to each YouTube url in the dataset is saved to text file and frame wise time stamps are removed.

OpenAI Whisper ASR, the other model which we have used to investigating bias have made public the following five pre-trained model variants through the API hosted at GitHub.


\begin{table}[ht]
\caption{Details of the available OpenAI Whisper models and their approximate memory requirements and relative performance 
on a sample dataset of 100 audio files}
\label{tab:my-table}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Model Name}} & \multicolumn{1}{l|}{\textbf{Parameters}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Required\\ VRAM\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Avg\\ Inference\\ Time\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Avg\\ WER\end{tabular}}} \\ \hline
tiny.en & 39 M & $\sim$1 GB & 1.2 min &  \\ \hline
base.en & 74 M & $\sim$1 GB & 1.6 min &  \\ \hline
small.en & 244 M & $\sim$2 GB &  &  \\ \hline
medium-en & 769 M & $\sim$5 GB &  &  \\ \hline
large & 1550 M & $\sim$10 GB &  &  \\ \hline
\end{tabular}
\end{table}

For generating the transcripts using OpenAI Whisper ASR model, we have download the videos using python API YT DLP ~\cite{pypiYtdlp} and extract audio in mp3 format from it using ffmpeg library,.used the pre-trained base model (base.en) of OpenAI Whisper ASR which is trained on English corpus.We have made this choice as base model performance is optimal for our dataset in terms of accuracy and inference time. On an average, each lecture is of approximately 50 minutes and it took an inference time of 1-2 minutes on a server having Tesla P100 PCIe 16 GB GPU. To run the inference on entire audio dataset using Open AI Whisper base.en model, the time taken is around 250 hours as transcription generation process is run on  two GPU servers in parallel.

\subsection{Dataset statistics}
The curated TIE dataset consists of 9860 audio files accounting for approximated 8740 hours of speech and 62M word utterances from 321 speakers  along with their ground truth , ASR generated transcripts using YouTube Captions and OpenAI Whisper model. For each lecture, we have metadata corresponding to speaker and lecture content labelled. We do have multiple audio samples for each speaker to account for variation in audio topic content and presence of noise in audio signal. The detailed statistics of the dataset is tabulated in Table 1:



\begin{table}[ht]
\caption{Dataset statistics corresponding to labelled attributes}
\label{tab:my-table}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Attribute}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Attribute\\   Subgroups\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}No. of \\  Speakers\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}No. of \\  Videos\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}No. of \\  Hours\end{tabular}}} \\ \hline
\multirow{2}{*}{Gender} & Female & 17 & 569 & 498 \\ \cline{2-5} 
 & Male & 315 & 9291 & 8242 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Caste\\  Category\end{tabular}} & Reserved & 92 & 2662 & 2285 \\ \cline{2-5} 
 & Unreserved & 243 & 7198 & 6455 \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Seniority\\  Level\end{tabular}} & Very Senior & 47 & 1349 & 1238 \\ \cline{2-5} 
 & Senior & 78 & 2231 & 1943 \\ \cline{2-5} 
 & Junior & 109 & 3346 & 3033 \\ \cline{2-5} 
 & Very Junior & 99 & 2934 & 2526 \\ \hline
\multirow{3}{*}{Speech rate} & Slow & 242 & 3851 & 3442 \\ \cline{2-5} 
 & Average & 237 & 2118 & 1880 \\ \cline{2-5} 
 & Fast & 250 & 3891 & 3418 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Discipline \\ Group\end{tabular}}} & \multicolumn{1}{l|}{Engineering} & 238 & 6976 & 6269 \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Non-\\ Engineering\end{tabular}} & 103 & 2884 & 2472 \\ \hline

\end{tabular}
\end{table}

As it can be seen from the from the statistics that the  gender representation is highly skewed in favor of males(95\%) compared to females(5\%) . It is to be noted that we have sampled this dataset from NPTEL in which lecturers from premier Indian engineering institutes (IITs \footnote{https://en.wikipedia.org/wiki/Indian\_Institutes\_of\_Technology})  deliver lecture series on different subjects. Studies like ~\cite{prathap2017excellence,chanana2006gender} have highlighted the marginalized representation of females in teaching and leadership profiles in Indian Higher Education institutions.Also as per All Indian Survey on Higher Education (AISHE) \footnote{https://aishe.gov.in/} latest report published for financial year 2019-20, the gender distribution at different positions of teaching hierarchy in Institute of National Importance \footnote{https://en.wikipedia.org/wiki/Institutes\_of\_National\_Importance} is as follows

\begin{table}[ht]
\caption{ Distribution of Teachers across demographic traits in Institute of National Importance for reference period 2019-20}
\label{tab:my-table}
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Total No. of  \\ Teachers\end{tabular}} & 17282 \\ \hline
\textbf{Female Share(\%)} & 20.3 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Reserved Caste \\ Category Share (\%)\end{tabular}} & 21.0 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Professor and\\ Equivalent Share (\%)\end{tabular}} & 29.4 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Associate \\ Professor Share (\%)\end{tabular}} & 24.6 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Assistant \\ Professor Share (\%)\end{tabular}} & 46.0 \\ \hline
\end{tabular}
\end{table}

The imbalance in distribution of lecturers as actually present in premier engineering institutes across gender, reserved caste category and seniority is reflected in our dataset too. We also tried to study the intersection of attributes to understand how they interact with each other. The share of female in different groups is tabulated below:

\begin{table}[ht]
\caption{Females share (\%)  across labelled groups}
\label{tab:my-table}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Attribute}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Attribute\\   Subgroups\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Speakers\\ Share (\%)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Videos\\ Share(\%)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Hours\\ Share(\%)\end{tabular}}} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Caste\\  Category\end{tabular}} & Reserved & 2.2 & 3.8 & 3.4 \\ \cline{2-5} 
 & Unreserved & 6.6 & 6.5 & 6.5 \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Seniority\\  Level\end{tabular}} & Very Senior & 4.3 & 7.1 & 6.8 \\ \cline{2-5} 
 & Senior & 5.1 & 6.9 & 6.3 \\ \cline{2-5} 
 & Junior & 1.8 & 1.6 & 1.7 \\ \cline{2-5} 
 & Very Junior & 10.0 & 9.1 & 9.5 \\ \hline
\multirow{3}{*}{Speech rate} & Slow & 5.0 & 4.3 & 4.3 \\ \cline{2-5} 
 & Average & 5.5 & 7.3 & 6.9 \\ \cline{2-5} 
 & Fast & 6.4 & 6.4 & 6.5 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Discipline \\ Group\end{tabular}}} & \multicolumn{1}{l|}{Engineering} & 1.7 & 2.0 & 1.9 \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Non-\\ Engineering\end{tabular}} & 14.6 & 14.9 & 15.4 \\ \hline
\end{tabular}
\end{table}

\begin{table}[ht]
\caption{Reserved caste category share (\%)  across labelled groups}
\label{tab:my-table}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Attribute}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Attribute\\   Subgroups\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Speakers\\ Share (\%)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Videos\\ Share(\%)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Hours\\ Share(\%)\end{tabular}}} \\ \hline
\multirow{2}{*}{Gender} & Female & 11.1 & 17.9 & 15.4 \\ \cline{2-5} 
 & Male & 28.3 & 27.6 & 26.8 \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Seniority\\  Level\end{tabular}} & Very Senior & 29.8 & 23.1 & 23.3 \\ \cline{2-5} 
 & Senior & 29.5 & 36.3 & 33.9 \\ \cline{2-5} 
 & Junior & 28.4 & 27.8 & 27.2 \\ \cline{2-5} 
 & Very Junior & 23.5 & 20.9 & 20.3 \\ \hline
\multirow{3}{*}{Speech rate} & Slow & 25.6 & 26.5 & 25.8 \\ \cline{2-5} 
 & Average & 26.2 & 30.5 & 29.6 \\ \cline{2-5} 
 & Fast & 28.1 & 25.5 & 24.6 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Discipline \\ Group\end{tabular}}} & \multicolumn{1}{l|}{Engineering} & 29.1 & 28.3 & 27.9 \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Non-\\ Engineering\end{tabular}} & 23.8 & 23.8 & 21.6 \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\caption{Seniority wise number of speakers share (\%)  across labelled groups}
\label{tab:my-table}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Attribute}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Attribute\\  Subgroups\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Very \\ Senior\\ Share\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Senior\\ Share\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Junior\\ Share\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Very \\ Junior\\ Share\end{tabular}}} \\ \hline
\multirow{2}{*}{Gender} & Female & 11.1 & 22.2 & 11.1 & 55.6 \\ \cline{2-6} 
 & Male & 14.2 & 23.4 & 33.9 & 28.5 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Caste \\ Category\end{tabular}} & Reserved & 15.2 & 25.0 & 33.7 & 26.1 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}Un-\\ reserved\end{tabular} & 13.5 & 22.5 & 32.0 & 32.0 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Speech \\ rate\end{tabular}} & Slow & 14.8 & 24.7 & 32.9 & 27.6 \\ \cline{2-6} 
 & Average & 15.1 & 23.1 & 34.5 & 27.3 \\ \cline{2-6} 
 & Fast & 13.2 & 21.2 & 35.6 & 30.0 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Disci-\\ pline \\ Group\end{tabular}}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Engi-\\ neering\end{tabular}} & 14.5 & 24.4 & 38.0 & 23.1 \\ \cline{2-6} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Non- Engi-\\ neering\end{tabular}} & 13.6 & 21.4 & 21.4 & 43.7 \\ \hline
\end{tabular}
\end{table}
\subsection{Evaluation metric}
After having the labelled dataset along with ground-truth, YouTube Captions and OpenAI Whisper transcripts, we need to have an evaluation metric that can be used to compare performance of both ASRs. There are several metrics that are commonly used to evaluate the performance of an automatic speech recognition (ASR) system. Some of the most common metrics include:
\begin{itemize}
    \item Word error rate (WER): This is the most commonly used metric for evaluating ASR performance. It is defined as the percentage of words that are incorrectly recognized by the system.
    \item Perplexity: This is a measure of how well the ASR system is able to predict the next word in a sequence, given the previous words. A lower perplexity indicates better performance.
    \item Character error rate (CER): This is similar to WER, but it is based on the number of incorrectly recognized characters rather than words.
    \item Word accuracy: This is the percentage of words that are correctly recognized by the system.
    \item Confusion matrix: This is a matrix that shows the number of times each word was incorrectly recognized as a different word.
    
\end{itemize}

Some of the recent works like ~\cite{https://doi.org/10.48550/arxiv.2209.10591} and ~\cite{https://doi.org/10.48550/arxiv.2104.02138} have proposed BERTScore and SemDist measures focusing on semantic closeness of ground-truth sentences and ASR generated sentences.However, we have chosen WER as an evaluation metric for this work of ours due to to the following reasons:
\begin{itemize}
    \item WER is easy to understand and interpret: It is a simple percentage that represents the number of words that are incorrectly recognized by the system.
    \item WER is widely used: It is the most commonly used metric for evaluating ASR performance, which means that there is a lot of data available for comparison purposes.Most of the bias literature in ASR ~\cite{Tatman2017EffectsOT,tatman-2017-gender,racial_dispar,252643719} have used it for reporting disparities among groups. In addition, WER is widely used as benchmarking metric by ASR models on different public datasets.  
    \item WER is sensitive to errors: It takes into account all types of errors, including insertion, deletion, and substitution errors as WER is defined as  \[WER =  \frac{S+D+I}{N}  \], where S,D and I are the number of substitutions, deletions
and insertions needed to transform the reference text into the hypothesis text, while N is the number of words in the reference text.This makes it a good metric for identifying areas where the ASR system needs to be improved.
    \item WER can be easily computed: It is straightforward to calculate WER from the transcriptions produced by the ASR system and a reference transcription. For a large corpus of 9860 transcripts having an average of 5000 words to be compared against to transcripts generated by YouTube Caption and OpenAI Whisper AI , WER is best suited
\end{itemize}

We measure the WER in two steps, a preprocessing step  in which we alter the reference ground truth and the ASR generated text to  WER calculation step to reduce the occurrence of false mis-transcriptions due to the presence of equivalent but different, words and a WER calculation step, in which we calculate the WER directly using the JiWER ~\cite{Jiwer_LIB} Python library.


\subsection{Bias Determination}
After we have calculated the WER for both of the ASR generated transcripts against the ground truth transcripts for each lecture,  we measure how the WER varies  with respect to each platform , each discipline and each speaker characteristic.We conclude bias is present in the ASR for any speaker demographic or lecture content attribute , if we find statistically significant difference in WER within the subgroups defined by the given attribute.For example, if a ASR platform has a WER which is consistently and significantly lower for females when compared to males, we can say that the platform is exhibiting bias corresponding to gender attribute of speaker.

As it is evident from the figure 1 below  WER distribution for both ASR under investigation is not normal.

\begin{figure}
    \centering
    \includegraphics{error_rate_plot.pdf}
    \caption{WER Distribution of YouTube and OpenAI Whisper ASR}
    \label{fig:my_label}
\end{figure}




We have also performed Shapiro–Wilk test $(\alpha = 0.001)$ for normality over both of the distribution and found the ShapiroResult(statistic=0.90791, pvalue=0.0) and ShapiroResult (statistic=0.787, pvalue\textless 0.00001)  for YouTube Captions and OpenAI Whisper  WER distribution respectively. The result confirms that both of the distribution are non-normal and hence parametric statistical tests like paired t-test or ANOVA will not be helpful in drawing any conclusion over the given distributions. Hence, we have used non-parametric statistical test Kruskal Wallis $(\alpha = 0.001)$ using which we will determine whether there is a significant difference between the medians of two or more groups based on the demographic or non-demographic set of attributes.

==> Experiments.tex <==
\subsection{Evaluation metric}
After having the labelled dataset along with ground-truth, YouTube Captions and OpenAI Whisper transcripts, we need to have an evaluation metric that can be used to compare performance of both ASRs. 

There are several commonly used metrics like Word Error Rate(WER) , Character error rate (CER) , Perplexity etc. Some of the recent works like ~\cite{https://doi.org/10.48550/arxiv.2209.10591} and ~\cite{https://doi.org/10.48550/arxiv.2104.02138} have proposed BERTScore and SemDist measures focusing on semantic closeness of ground-truth sentences and ASR generated sentences.However, we have chosen WER as an evaluation metric for this work of ours due to to the following reasons:
\begin{itemize}
    \item WER is easy to understand and interpret: It is a simple percentage that represents the number of words that are incorrectly recognized by the system.
    \item WER is widely used: It is the most commonly used metric for evaluating ASR performance, which means that there is a lot of data available for comparison purposes.Most of the bias literature in ASR ~\cite{Tatman2017EffectsOT,tatman-2017-gender,racial_dispar,252643719} have used it for reporting disparities among groups. In addition, WER is widely used as benchmarking metric by ASR models on different public datasets.  
    \item WER is sensitive to errors: It takes into account all types of errors, including insertion, deletion, and substitution errors as WER is defined as  \[WER =  \frac{S+D+I}{N}  \], where S,D and I are the number of substitutions, deletions
and insertions needed to transform the reference text into the hypothesis text, while N is the number of words in the reference text.This makes it a good metric for identifying areas where the ASR system needs to be improved.
    \item WER can be easily computed: It is straightforward to calculate WER from the transcriptions produced by the ASR system and a reference transcription. For a large corpus of 9860 transcripts having an average of 5000 words to be compared against to transcripts generated by YouTube Caption and OpenAI Whisper AI , WER is best suited
\end{itemize}

We measure the WER in two steps, a preprocessing step  in which we alter the reference ground truth and the ASR generated text to  WER calculation step to reduce the occurrence of false mis-transcriptions due to the presence of equivalent but different, words and a WER calculation step, in which we calculate the WER directly using the JiWER ~\cite{Jiwer_LIB} Python library.

\subsection{Bias Determination}
After we have calculated the WER for both of the ASR generated transcripts against the ground truth transcripts for each lecture,  we measure how the WER varies  with respect to each platform , each discipline and each speaker characteristic.We conclude bias is present in the ASR for any speaker demographic or lecture content attribute , if we find statistically significant difference in WER within the subgroups defined by the given attribute.For example, if a ASR platform has a WER which is consistently and significantly lower for females when compared to males, we can say that the platform is exhibiting bias corresponding to gender attribute of speaker.

As it is evident from the figure 1 below  WER distribution for both ASR under investigation is not normal.

\begin{figure}
    \centering
    \includegraphics{error_rate_plot.pdf}
    \caption{WER Distribution of YouTube and OpenAI Whisper ASR}
    \label{fig:my_label}
\end{figure}




We have also performed Shapiro–Wilk test $(\alpha = 0.001)$ for normality over both of the distribution and found the ShapiroResult(statistic=0.90791, pvalue=0.0) and ShapiroResult (statistic=0.787, pvalue\textless 0.00001)  for YouTube Captions and OpenAI Whisper  WER distribution respectively. The result confirms that both of the distribution are non-normal and hence parametric statistical tests like paired t-test or ANOVA will not be helpful in drawing any conclusion over the given distributions. Hence, we have used non-parametric statistical test Kruskal Wallis $(\alpha = 0.001)$ using which we will determine whether there is a significant difference between the medians of two or more groups based on the demographic or non-demographic set of attributes.

==> introduction_new.tex <==
\section{Introduction}
Automatic speech recognition (ASR) technology, allowing users to provide voice based inputs to computing platforms, has been an active area of research since the 1950s. One of the most significant developments came in 2017 with the success of speaker independent voice recognition, with Microsoft~\cite{xiong2017the} reporting a \textit{word error rate} as low as 5.1\% on the 2000 Switchboard evaluation set. It not only reduces the typing effort for the individual, but also provides an alternate accessibility option for individuals who cannot use touch based interfaces. While speech recognition itself is useful for interacting with any digital device, it has also been integrated into voice assistants on mobile devices and, video sharing and video telephony platforms. The COVID-19 pandemic led to an increase in use of and research into this technology as it allowed individuals to interact with their devices without having to touch them.

\subsection{Learning through video lectures}
Since the early days of the COVID-19 pandemic, classrooms have shifted to an online mode with students attending lectures on video telephony platforms like Zoom and Google Meet. Another highly preferred platform used by students as a learning medium is YouTube which has course video lessons of various MOOC programs like edX ~\cite{edxFreeOnline}, MIT OCW~\cite{ocw2008opencourseware}, NPTEL~\cite{krishnan2009nptel}, etc. and provides high quality educational content for free to students all around the world. This tectonic shift in learning pedagogy has a significant impact on how students consume knowledge, with the e-learning sector now growing at an unprecedented pace~\cite{wef_covid_online}. Research has shown students preferring video-based e-learning, either through live lectures~\cite{MUTHUPRASAD2021100101} or pre-recorded lecture videos~\cite{syynimaa2019does} to in-person classes. \cite{islam2020_zoompre} showed that students may also prefer pre-recorded videos to live online classes. 

\subsection{Pre-recorded video lectures}
YouTube lecture videos are a unidirectional mode of communication and often delivered by instructors for whom English is a non-native language. For example, the NPTEL (National Programme on Technology Enhanced Learning) MOOC YouTube channel has over 2 million subscribers and is the most viewed educational content channel in the world. Lectures on this channel are disseminated by instructors from various premier educational institutes of India (IITs and IISc), all of whom are non-native English speakers. Thus, while it is essential to ensure proper pronunciation, clear diction, and a neutral accent to avoid a negative impact on the learning outcome or on the instructor feedback, this cannot always be guaranteed. Video captions can be used to alleviate some of these concerns, but the average length of an educational lecture may be upwards of 50 minutes and it may not be always possible for the instructor to transcribe the video lecture themselves. \cite{Chan2022} showed that incorrect captions may have an impact on the learning ability of the students. %\sjnote{IMP: Prior literature shows that accent does not impact learning outcomes but may impact perception of the instructor.}

\subsection{Automatic caption generation}
ASRs can bridge this gap by ingesting the speaker's voice as input and automatically generating captions synced with the video. There are multiple platforms like YouTube~\cite{Youtube_Live}, Zoom~\cite{Zoom_Live}, Otter.AI ~\cite{otterai}, etc. that generate automatic captions for audio/video files. These platforms are expected to work without disparity for all speaking rates, accents, tonality, independent of gender or age to ensure correct transcripts are generated and the listener does not misinterpret the speaker. While misunderstanding may not be as harmful for normal videos, it may seriously impact students watching educational content as it can have a direct impact on the learning outcome~\cite{willems2019increasing}.%\amnote{find some references discussing this.}\arnote{Can't find any. SJ can you please add some}

\subsection{Disparity in caption generation}
There has been ongoing research evaluating disparities in ASRs toward different racial~\cite{koenecke2020racial}, gender~\cite{tatman2017gender} and other groups~\cite{feng2021quantifying}. %due to differences in various attributes like gender, age, race/ethnicity, accents, and speech impairments. 
Most of these studies have focused on Western languages, accents, and social demographic groups. There have also been efforts to create public datasets like Artie Bias~\cite{meyer2020artie}, CORAAL~\cite{CORAAL}, AAVE~\cite{AAVE}, TED-LIUM~\cite{rousseau2012ted}, Librispeech~\cite{panayotov2015librispeech} etc., with dialectical and vernacular variations to evaluate the performance of existing ASR platforms, but these too have primarily focused on Western speakers. Moreover, there has been a lack of datasets exploring technical or pedagogical content.

\subsection{Use of ASRs in India}
Multiple studies in the literature have evaluated the accuracy of ASRs for native English speakers on non-educational content~\cite{tatman2017effects,tatman2017gender,koenecke2020racial}, but there has been a shortage of studies evaluating the performance of ASRs for non-native speakers, e.g., Indian speakers. Moreover, a significant number of students within India consume educational content from YouTube or other e-learning platforms~\cite{buddayya2019benefits}, but there have been no studies evaluating the transcription accuracy of ASRs for educational content delivered by Indian speakers. Due to the scale at which content is disseminated and consumed in India, it is important for researchers to study the disparities in widely deployed and state-of-the-art ASRs to ensure proper learning pedagogy is maintained.

In this study, we evaluate the correctness of captions for two popular ASR platforms -- YouTube Automatic Captions ~\cite{Youtube_Live} and OpenAI's Whisper ~\cite{radford2022robust} on a new large-scale dataset developed by us. This dataset, developed by us and called Technical Indian English (TIE), has more than 9800 educational videos from the NPTEL MOOC learning platform, comprising over 8700 hours of content and 62 million spoken words. These lecture videos are delivered by 332 speakers belonging to different gender, caste, age and regions within India. Ours is the first such annotated dataset on Indian educational videos and our in-depth analysis of the performance of the two ASRs on this dataset shows that disparities exist not only between the two platforms but also between categories like male vs female gender, old vs young age, etc. on each platform. While studies have been conducted to evaluate YouTube's ASR capabilities, ours is the first study to evaluate OpenAI's Whisper for its accuracy on technical English content, spoken by non-native English speakers.

We now list the research questions that we address in this study.

\noindent \textbf{RQ1.} Since no prior dataset exists for studying ASR disparities across educational videos for non-native speakers the first question we were faced with was to develop such a dataset from scratch. In response we built the TIE dataset.%\sjnote{do we add development of dataset as an RQ here?}

\noindent \textbf{RQ2.} How do the two ASRs perform on the TIE dataset? We perform statistical tests to identify which of the two platforms is better at transcribing technical educational content spoken by Indian speakers.

\noindent \textbf{RQ3.} Do the two ASR platforms exhibit disparity in performance between the different categories within each attribute like gender, caste, age, etc. Here as well we perform statistical tests to identify the disparities in performance not only for a given platform but also across platforms.

Finally, we list our contributions. In this paper, we propose the TIE dataset of 9860 audio files spanning a massive duration of 8740 hours worth of lectures sourced from the NPTEL MOOC platform and annotated for attributes corresponding to the lectures and the 332 instructors who have delivered these lectures. We believe that this dataset can serve as an excellent benchmark for studying the performance of various AI softwares including ASRs. We audit the YouTube Automatic Captions and OpenAI Whisper ASRs for existing disparities towards gender, caste, teaching experience, native region of the speakers, speech rate and, technical discipline of the lectures. 

Our analysis reveals a significant disparity against non-native English speakers in the Indian population, particularly for male speakers, speakers from southern India, and those with a slow speech rate. In addition, we found that the age of speakers and the topic of speech had an impact on the accuracy of ASRs. We also observed that while Whisper had better overall accuracy than YouTube, disparities were higher in Whisper. We conclude by discussing possible causes of these disparities and proposing strategies to address them.
%\amnote{Write the key observations from this analysis in a few lines.} \arnote{Done}

% \sjnote{Please add one paragraph of our contributions.} \arnote{Done}

% \sjnote{AR-- ADD ONE PARAGRAPH ON ``Ethics Statement''} 

\subsection{Broader perspective, ethics and competing interests}
ASR systems have been shown to have bias toward specific sub-population of society due to non-standard accent and dialects. For a linguistically diverse and vast population like India, bias of ASR systems may have serious consequences in providing equitable access to ASR based technologies. In this work, we evaluate disparities in two ASRs -- YouTube Automatic Captions and OpenAI Whisper -- on a self curated dataset of technical lectures, which is highly relevant from a pedagogical point of view in the Indian context. As online education has been an enabler in democratising education in developing economies like India, errors in ASR generated transcripts can seriously impact both lecture delivery of instructors and learning outcome of students~\cite{willems2019increasing}. %\amnote{Add reference}\arnote{Done}

This audit study and evaluation dataset will enable the ASR system developers in investigating and addressing the biases in these systems which disproportionately affect certain demographic groups. %However, the results may also lead to generalisation of disparities toward certain sections of society which may be untrue when evaluated against a more vast, diverse and representative dataset. 
However, if our dataset is used for training any ASR system, it may exhibit data bias due to skewed representation of some of the demographic attributes. Thus we advise practitioners to use caution with the same.

%We have highlighted the existing disparities in ASRs under investigation for under-represented groups corresponding to each demographic attribute of speaker. 
While annotating sensitive demographic attributes of the speakers like gender and caste in our dataset, we  specifically label them as perceived gender and perceived caste since self-identified gender and caste information were not available in the public domain. We take due care in anonymising the instructor name and associated institute name corresponding to each lecture to avoid individual level and institute level evaluation based on word error rates in future works.

==> methodology_old.tex <==
\section {Methodology}
\sjnote{Heavy rewrite required. Cannot add everything as a bulleted list. Need to have well defined paragraphs, figures to explain sequence diagram etc.}
The methodology used for the dataset curation , annotatation and testing of hypothesis is outlined in the below points:
\begin{itemize}
\item   To ensure the content diversity of the dataset and capturing the demographic representation of lecturers in Indian Higher Education Institutes, 10272 NPTEL video lectures have been added to our dataset.
\item   The use of YouTube-hosted NPTEL lectures has been motivated by the convenience and accessibility of the lectures along with their manual and YouTube Captions auto generated transcripts
\item   Word Error Rate (WER) has been chosen as an evaluation metric of transcription accuracy on the dataset not only because it is simple to understand and easy to compute but since OpenAI Whisper and other similar models have used this metric to benchmark their models
\item   To account for the ground truth errors like typing mistakes in manual transcripts, bottom 5\% and the top 5\% videos in terms of WER accuracy on have been removed from the dataset resulting the 9860 videos the final dataset used for further analysis
\item   For 332 distinct speakers from different domain an average of 30 lectures per speaker and 6300-word utterances per speaker has been taken of our dataset to understand whether the WER is due to diverse content or because of variation of utterances characterized by pitch, loudness, sample rate and other auditory features
\item   Each lecture duration is 1 hour on average with manual transcript corpus length of entire dataset being 62M words to help us investigate the coverage of language model of both ASRs
\item   The metadata of the video which includes Course Name, Discipline Name, Institution Name, Instructor Name and YouTube URL has been scrapped from the NPTEL website
\item   Instructors Gender, Native State and Year of Joining the Institute has manually annotated with the information sourced from their home pages hosted on their respective Institute Website, Google Scholar, Infibnet websites etc. Computer-assisted and unassisted lecture videos have also been annotated manually.
\item Manual and YouTube Captions Auto-Generated Transcripts in English have been downloaded from YouTube using YouTubeTranscript API in python
\item   Using the Youtube DL library duration of each video has been sourced and Speech Rate attribute corresponding to each video is derived from number of words in manual transcript and duration of video
\item   Audio corresponding to each video has been extracted and downloaded from the YouTube using YT\_ DLP API and FFMPEG library 
\item   Open AI Whisper base model has been used to generate transcripts from the downloaded audios corresponding to each video in the dataset.
\item   Number of out of vocabulary (OOV) words in manual transcript of each video corresponding to corpus of YouTube Captions and OpenAI Whisper generated transcripts has also been used a feature to understand correlation of WER and number of OOV words
\item   To investigate the bias in transcription accuracy at modular level of both ASRs , features annotated and derived are divided into two sets. Gender, Speech Rate, Native Region , Age Group , Assisted lectures features which represents implicit speech variation are used for bias estimate in acoustic model of ASR. No. of OOV Words, Discipline , Type Token Ratio (TTR) are used for evaluating bias estimate in language model of both ASRs
\item   Keeping in view, the non-normal distribution of WER of both ASR, Man-Whitney U test is used for binary features, while Kruskal-Wallis Test is used for non-binary features to test our null hypothesis that WER is independent of any feature group.
\item   As the dataset used is unbalanced or skewed for certain features, stratified sampling is used before hypothesis testing with a significance level of 0.0001 for accepting/rejecting any null hypothesis.

\end{itemize}


==> results.tex <==
\section{Results}
We now present the results from our experimental evaluation of the YouTube and Whisper ASRs' transcriptions for the TIE dataset. We first evaluate the overall performance of the two platforms, followed by an in-depth study of the disparities between the different categories for each demographic attribute and speech characteristic mentioned in Table~\ref{tab:dataset_metadata}.

% In this section we investigate the difference in  WER among YouTube Caption and OpenAI Whsiper ASR due to variability in speaker demographic and speech characteristics. We will also look if there is a difference in WER due to content diversity among both of the ASRs.

\subsection{Overall Disparity}
From Figure~\ref{fig:histogram_wer}, we see that for the YouTube platform, only 75.6\% videos have a Word Error Rate (WER) lower than 0.2 whereas this ratio is 84.0\% for Whisper's ASR transcriptions. This indicates that on average, Whisper reports lower errors in transcription compared to Youtube. However, Whisper also reports a WER as high as Y.Y for XX\% of the videos, which we consider as outliers. To better understand the differences in the WER distribution of both ASRs, we look at Figure~\ref{fig:overall_boxplot_wer} which does not feature the outlier data points.

% Before going into results of bias determination in ASRs due to speaker and speech characteristics, we would like to understand baseline difference in WER of both ASRs.As we can visualize from the Figure 1, WER distribution OpenAI Whisper there are higher number of speech lectures that fall into low WER bins than that of YouTube Captions, indicating its better performance than YouTube Captions. However the spread  of bins from 0 to 1 in WER distribution of OpenAI Whisper indicates presence of outliers. The difference in WER distribution of both ASRs is more evident in the below boxplot which is plotted by removing outliers from WER distributions of ASRs. 

\begin{figure}[!t]
    \centering
    \includegraphics[width= 0.75\columnwidth, width =3cm, keepaspectratio]{figures/overall_WER.pdf}
    \caption{Boxplot distribution of the Word Error Rate (WER) for Youtube(YTB) and Whisper(WSPR) ASRs on the TIE dataset.\sjnote{add one line on insight from figure}}
    \label{fig:overall_boxplot_wer}
\end{figure}

From Figure~\ref{fig:overall_boxplot_wer}, we see that Whisper's median WER is 12\%, and this is significantly less ($H$ = 803.88, $p$-value $\leq$ 0.001) than YouTube's WER at 14 \%. This indicates that Whisper's base model outperforms YouTube in terms of overall performance on the TIE dataset. We also notice that YouTube has higher maximum WER (XX \%) compared to Whisper (XX \%), thus confirming the worse performance of YouTube. This can be attributed to the Whisper zero-shot transcription model which is trained on a large corpora better generalizes on the given dataset. \sjnote{Is this confirmed or assumption? Should not put in if assumption.}

% It can be seen  median of OpenAI Wisper is 12  percent which is significantly lower ((H=803.88, $pvalue \leq 0.001$) than the median of YouTube Captions ASR WER distribution which is 14 percent. This indicates that OpenAI Whisper base model outperforms YouTurbe Captions on the TIE dataset which can be attributed to the Whisper zero-shot transcription model which is trained on a large corpora better generalizes on the given dataset.But without knowing the training dataset of YouTube Captions it cannot be affirmatively stated.

On analysing the lecture wise WER of both models, it is found that errors of both models are strongly correlated with correlation coefficient of 0.81 indicating WER of both models follow a pattern for a given set of inputs.However, it's quite possible that both models have different strengths and weaknesses, and perform differently on different datasets. WE will analyse impact of speaker and speech characteristics on WER of each model separately in upcoming subsections. \sjnote{is there a figure to show this correlation? what do you mean by lecture wise WER? } 

\begin{table}[!t]
    \small
    \centering
    \begin{tabular}{|c|c|c|l|}
    \hline
     \textbf{Category} & \textbf{Attribute} & \textbf{WER (\%)} & \textbf{Test}\sjnote{what test?}\\
     \hline
     \multirow{2}{*}{\textbf{Gender}} & Female & 13.6 & \multirow{2}{*}{$H$ = 23.3, $p$ \textless 0.001} \\
     \cline{2-3}
     & Male & \textbf{14.5} & \\ 
     \hline\hline
     \multirow{2}{*}{\textbf{Caste}} & RES & 13.8 & \multirow{2}{*}{$H$ = 15.2, $p$ \textless 0.001} \\
     \cline{2-3}
     & UR & \textbf{14.6} & \\ 
     \hline\hline
     \multirow{4}{*}{\textbf{Exp.}} & $\leq$ 1980 & \textbf{15.9} & \multirow{4}{*}{$H$ = 125.8, $p$ \textless 0.001} \\
     \cline{2-3}
     & 1981-90 & 13.3 & \\ 
     \cline{2-3}
     & 1991-00 & 14.9 & \\ 
     \cline{2-3}
     & $\geq$ 2001 & 14.0 & \\ 
     \hline\hline
     \multirow{4}{*}{\textbf{Native}} & North & 13.6 & \multirow{4}{*}{$H$ = 80.9, $p$ \textless 0.001} \\
     \cline{2-3}
     & South & \textbf{15.4} & \\ 
     \cline{2-3}
     & East & 14.2 & \\ 
     \cline{2-3}
     & West & 14.4 & \\ 
     \hline\hline
     \multirow{3}{*}{\textbf{Speech Rate}} & Slow & \textbf{15.3} & \multirow{3}{*}{$H$ = 104, $p$ \textless 0.001} \\
     \cline{2-3}
     & Avg. & 14.2 & \\ 
     \cline{2-3}
     & Fast & 13.9 & \\ 
     \hline\hline
    \multirow{2}{*}{\textbf{Discipline}} & Non-Eng. & 13.5 & \multirow{2}{*}{$H$ = 110.8, $p$ \textless 0.001} \\
     \cline{2-3}
     & Engg. & \textbf{14.8} & \\ 
     \hline
    \end{tabular}
    \caption{Word Error Rate (WER) and XX Test\sjnote{what test?} results for transcripts generated by YouTube Automatic Captions ASR. \sjnote{should we combine YTB and WSPR in a single table?}}
    \label{tab:yt_comparison_tbl}
\end{table}

\subsection{YouTube Automatic Captions}
We now look at the YouTube ASR performance for transcript generation across various demographic and non-demographic attributes.

% We will explore the YouTube ASR model performance across various demographic and non-demographic attributes of speaker in upcoming sub-sections.

% \begin{table}[t]
% \begin{tabular}{|c|c|c|l|}
% \hline
% \multicolumn{1}{l}{\textbf{Category}} & \multicolumn{1}{l}{\textbf{Attribute}} & \multicolumn{1}{l}{\textbf{WER (\%)}} & \multicolumn{1}{c}{\textbf{Test Result}} \\ \hline
% \multirow{2}{*}{\textbf{Gender}} & Female & 13.6 & \multicolumn{1}{c}{\multirow{2}{*}{H=23.3,p\textless{}0.001}} \\
%  & Male & 14.5 & \multicolumn{1}{c}{} \\ \hline
% \multirow{2}{*}{\textbf{Caste}} & RES & 13.8 & \multicolumn{1}{c}{\multirow{2}{*}{H=15.2, p\textless{}0.001}} \\
%  & UR & 14.6 & \multicolumn{1}{c}{} \\ \hline
% \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Teaching \\ Since\end{tabular}}} & \textless{}=1980 & 15.9 & \multicolumn{1}{c}{\multirow{4}{*}{H=125.8,p\textless{}0.001}} \\
%  & 1981-90 & 13.3 & \multicolumn{1}{c}{} \\
%  & 1991-00 & 14.9 & \multicolumn{1}{c}{} \\
%  & \textgreater{}=2001 & 14.0 & \multicolumn{1}{c}{} \\ \hline
% \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Native\\ Region\end{tabular}}} & East & 14.2 & \multirow{4}{*}{H=80.9,p\textless{}0.001} \\
%  & West & 14.4 &  \\
%  & North & 13.6 &  \\
%  & South & 15.4 &  \\ \hline
% \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Speech \\ Rate\end{tabular}}} & Slow & 15.3 & \multirow{3}{*}{H=104,p\textless{}0.001} \\
%  & Average & 14.2 &  \\
%  & Fast & 13.9 &  \\ \hline
% \multicolumn{1}{l}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Discipline\\ Group\end{tabular}}}} & Non-Eng. & 13.5 & \multirow{2}{*}{H=110.8,p\textless{}0.001} \\
% \multicolumn{1}{l}{} & Eng. & 14.8 &  \\ \hline
% \end{tabular}
% \caption{Results on YouTube Automatic Captions}
% \label{tab:yt_comaparison_tbl}
% \end{table}

% \begin{figure*}[t]
% 	\begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=2.5cm, keepaspectratio]{figures/gender_yt.pdf}
% 		\caption{Gender}
% 		\label{fig:yt_gender}
% 	\end{subfigure}\hfill%
% 	~\begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=2.3cm, keepaspectratio]{figures/caste_yt.pdf}
% 		\caption{Caste}
% 		\label{fig:yt_caste}
% 	\end{subfigure}%
% 	~\begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=2.5cm, keepaspectratio]{figures/age_yt.pdf}
% 		\caption{Experience}
% 		\label{fig:yt_exp}
% 	\end{subfigure} \\
%     \begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=2.5cm, keepaspectratio]{figures/region_yt.pdf}
% 		\caption{Native Region}
% 		\label{fig:yt_native}
% 	\end{subfigure}\hfill% \hspace{2}
% 	~\begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=2.5cm, keepaspectratio]{figures/speech_yt.pdf}
% 		\caption{Speech Rate}
% 		\label{fig:yt_speed}
% 	\end{subfigure}
% 	~\begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=2.5cm, keepaspectratio]{figures/discipline_yt.pdf}
% 		\caption{Discipline}
% 		\label{fig:yt_discipline}
% 	\end{subfigure}
% 	\caption{WER Disparity across various attributes for YouTube Automatic Captions }
% 	\label{fig:word_error_rate}
% \end{figure*}


\begin{figure*}[t]
    \centering
	~\begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/gender_yt.pdf}
		\caption{Gender}
		\label{fig:yt_gender}
	\end{subfigure}%
	~\begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/caste_yt.pdf}
		\caption{Caste}
		\label{fig:yt_caste}
	\end{subfigure}%
	~\begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/age_yt.pdf}
		\caption{Experience}
		\label{fig:yt_exp}
	\end{subfigure} 
    \begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/region_yt.pdf}
		\caption{Native Region}
		\label{fig:yt_native}
	\end{subfigure}
	~\begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/speech_yt.pdf}
		\caption{Speech Rate}
		\label{fig:yt_speed}
	\end{subfigure}
	~\begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/discipline_yt.pdf}
		\caption{Discipline}
		\label{fig:yt_discipline}
	\end{subfigure}
	\caption{WER Disparity across various attributes for YouTube Automatic Captions }
	\label{fig:yt_word_error_rate}
\end{figure*}


\subsubsection{Gender Disparity}\sjnote{should we have disparity in title?}
\if{0}
It has been observed that the difference in median WER values due to gender attribute of speaker is 0.9\% . And the model is favoring the female voices compared to male voices (H=23.3,$p\leq 0.001$) , with median WER for female speakers being 13.6\% while for male speakers it is 14.5\%.From \ref{fig:yt_word_error_rate_a}, it can also also be concluded that the Youtube ASR model is consistently better for female voices as the Inter Quartile Range(IQR) for female voices 6.6\% compared to 9.3\% for males.
\fi

We compare the Word Error Rates (WER) between male and female speakers in the TIE dataset. Even though the dataset has more than 95\% male speakers, we notice that female speakers report lower median WER from Table~\ref{tab:yt_comparison_tbl} (difference of 0.9\%) and the XX-test's null hypothesis can be rejected \sjnote{add why we reject null hypothesis}. Next, looking at the boxplot distribution in Figure~\ref{fig:yt_gender}, we notice that males not only have have a higher WER (XX\%), but also a larger IQR as compared to female speakers.

% The results for disparity towards gender attribute by YouTube ASR are surprising as previous gender specific black box audits of YouTube Automatic Captions ~\cite{tatman2017effects} has reported no significant difference due to gender attribute and ~\cite{tatman2017gender} has stated that the model is performing better on male voices respectively, while benchmarking the model on white English Speakers dataset.

\noindent \paragraph{Takeaways:} On comparing male speakers against females, it can be inferred that--
\begin{itemize}
   \item WER for female voices is significantly lower (WER median difference = 0.9\%) than that of males, thus indicating a disparity between the transcripts for the two genders.
    \item The YouTube Automatic Captions performs consistently better for female voices than males.
\end{itemize}

\if{0}

\begin{table}[ht]
\caption{}
\label{gender_yt_table}
\begin{tabular}{lccc}
\hline
Category & \multicolumn{1}{l}{Atrribute} & \multicolumn{1}{l}{{Median  WER(\%)} & \multicolumn{1}{l}{Test Result} \\ \hline
Gender & Female & 6.6 & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}H= 23.3, \\ p\textless 0.001\end{tabular}} \\
 abc & Male & 9.3 & 
\\ \hline
Female & 13.6 & 6.6 & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}H= 23.3, \\ p\textless 0.001\end{tabular}} \\
Male & 14.5 & 9.3 & 

\end{tabular}
\end{table}

\fi

\subsubsection{Caste Disparity}
\if{0}
On comparing how caste category of speakers affected YouTube Automatic Captions performance, we observed a significant median difference(H=15.2,$p\leq 0.001$) of 0.8\% ,with reserved caste category speakers having low WER(median WER=13.8\%) compared to unreserved caste category speakers(median WER=14.6\%).
\fi

On comparing the performance of speakers belonging to Reserved castes against Unreserved castes, we note from Table~\ref{tab:yt_comparison_tbl}, a significant median difference ($H$ = 15.2, $p\leq$ 0.001) of 0.8\%, with Reserved caste speakers having low WER (median WER = 13.8\%) compared to unreserved caste speakers (median WER = 14.6\%). From Figure~\ref{fig:yt_caste}, we see that the distributions are fairly similar but Unreserved speakers report a slightly higher maximum WER at XX\%.

% Historically,Reserved caste category are under-privileged section of Indian society. The same has not been reflected in YouTube ASR performance while in Western Context, ~\cite{koenecke2020racial} has shown racial disparity against black speakers in Google ASR transcription.

\noindent \paragraph{Takeaways:}  On comparing the caste groups, it can be inferred that--
\begin{itemize}
   \item YouTube ASR performs relatively better for reserved caste category speakers. 
   \item The WER dispersion in both groups is similar indicating that the ASR is not able to clearly distinguish speakers from both groups.
\end{itemize}

\subsubsection{Experience Disparity}
% ~\cite{vipperla2010ageing} has pointed out age factor of speakers affects their speech recognition by ASR systems and the same  has also been reflected in our findings. 
We compare the performance of speakers belonging to different experience groups (a proxy for age) to understand how ASRs behave for speakers belonging to different age groups. From Table~\ref{tab:yt_comparison_tbl}, we notice that the worst performance is reported for the speakers with the most experience (WER = 16\%) and the best for speakers who started in the immediate next decade (WER = 13.3\%). Moreover, this difference is statistically significant ($H$ = 125.8, $p\leq$ 0.001). Figure~\ref{fig:yt_exp} shows that even though the median is lowest for speakers from 1981-90, the maximum is least for the youngest speakers (2001 onwards).

\noindent \paragraph{Takeaways:}  We now state the takeaways--
\begin{itemize}
   \item YouTube ASR performs best for speakers who started teaching between 1981-1990 and worst for those who started teaching before 1980. 
   \item YouTube ASR favors the young speakers as the Inter Quartile Range (IQR) reduces from 10.3\% to 7.8\% as we move from speakers with the most to the least experience (Fig~\ref{fig:yt_exp}).
\end{itemize}

\if{0}
\ref{fig:} show WER dispersion across experience of speakers grouped in four categories A($\leq 1980$ ), B(1981-90), C(1991-00) , D($\leq 01$). The IQR is lowest(7.8\%) for least  experienced speakers among four experience groups indicating the model's performance is more consistent with this group.

Age or experience of speakers has not been considered in any ASR related bias literature but our results show that age significantly (H=125.8,$p\leq 0.001$) impact YouTube Captions ASR with experience groups A,B, C and D having WER medians 15.9\%,13.3\%,14.9\% and 14.0\% respectively.
\fi

\subsubsection{Native Region Disparity}
We now study the change in the ASR performance based on the speaker's native region which may happen due to the regional accent. From Table~\ref{tab:yt_comparison_tbl}, we do not see any disparity between speakers hailing from West and East India, but the ASR performs best for speakers from North India (WER = 13.6\%) and worst for speakers from South India (WER = 15.4\%). Interestingly, the lowest IQR (\sjnote{add}) and maximum (XX \%) WER are reported for speakers from East India (Fig.~\ref{fig:yt_native}).
% Native region of speaker is a proxy for the regional accent of his speech and there have been many past work investigating impact of dialect or accent on ASR performance ~\cite{hinsvark2021_asrsurvey,tatman2017gender,tatman2017effects}.In sync with the previous works,our observations also state that regional accent variation of Indian English speakers impacts the ASR performance.

\noindent \paragraph{Takeaways:} The takeaways for the ASR performance based on the speakers' native region are--
\begin{itemize}
    \item The ASR reports a significant disparity between speakers from North India and other regions, but not between speakers from East and West India.
    \item The ASR reports the worst performance for speakers from South India.
   % \item The difference in WER median of West and East Indian Speakers is just 0.2\% indicating not disparity between these two groups.
   % \item However, YouTube ASR favors the North Indian speakers in comparison to speakers from all other regions with a stark WER median difference of 1.8\% between North and South Indian speakers. 
\end{itemize}

\if{0}
The variation of median WER which is 14.2\%, 14.4\%,13.6\% and 15.4\% for native speakers from East, West , North and South region respectively, may be attributed to the variation in Indian English accent of speakers.
\fi

\subsubsection{Speech Rate Disparity}
We now study the results for YouTube ASR for non-demographic attributes. In Table~\ref{tab:yt_comparison_tbl}, we see that interestingly, the slowest speakers have the worst WER (15.3\%) and the fastest speakers have the best WER (13.9\%). Figure~\ref{fig:yt_speed} shows a similar change in IQR and the maximum WER with an increase in speaking speed.
% It has been observed in our dataset which have multiple audio samples corresponding to each speaker that speech rate of each speaker varies from sample to sample. So the observed disparity(H=104.1,$p\leq 0.001$) in YouTube Captions due to speech rate category of lecture may not be fully attributed to speaker but also to the factors like lecture topic, preparedness of speaker etc.

\noindent \paragraph{Takeaways:} We have the following takeaways for YouTube ASR performance for speakers with different speech rates--
\begin{itemize}
   \item YouTube ASR is best in transcribing the audio files for speakers who speak the fastest. %belong to fast speech rate category
   \item The YouTube ASR performance becomes more consistent as we move from slow to fast speech rate (Fig.~\ref{fig:yt_speed}).
\end{itemize}

\if{0}
There is a WER median difference of 1.4\% favoring datapoints belonging to Fast Category(median WER 13.9\%) compared Average(median WER 14.2\%) and Slow(median WER 15.3\%) Speech Rate Category. As the distribution of the dataset corresponding to speech rate categoy is evenly distributed making the median difference even more significant.
\fi


\subsubsection{Discipline Disparity}
We divided the lecture videos into two disciplines-- Non-Engineering and Engineering, comprised of 23 different categories, to understand the performance of YouTube ASR for speech in different technical domains. From Table~\ref{tab:yt_comparison_tbl}, we can see that transcripts from Engineering discipline have a 1,3\% higher WER than those from Non-Engineering domain. This difference is statistically significant and thus a disparity exists between the two categories. From Figure~\ref{fig:yt_discipline}, we see that Engineering videos have a much higher maximum WER (XX \%) and a larger IQR.

% We categorized 23 different disciplines in Non-Engineering and Engineering Discipline Groups to understand the performance of YouTube ASR on domain specific speech datsets and the findings are summarized below:

\noindent \paragraph{Takeaways:}  We now list the takeaways for comparison between the two disciplines--
\begin{itemize}
   \item YouTube ASR performs better in lectures belonging to non-engineering category compared to the engineering category.
   \item YouTube ASR is better in generalizing for non-engineering domain datasets as the difference in IQR of both categories is 1.7\% (Fig.~\ref{fig:yt_discipline}).
\end{itemize}

% As the YouTube platform hosts a lot of technical lectures from speakers of Indian demography which is being consumed worldwide, the low generalization of its ASR model may impact the  effective lecture delivery process~\cite{kent2018case}

\if{0}

that there is disparity in its performance(H=110.8,$p\leq 0.001$) and it is performing better for non-engineering disciplines (median WER = 13.5\%) compared to engineering disciplines(median WER = 14.8\%).
\fi

% We have also analysed how the YouTube ASR perform on the intersection of few features, which may be considered independent of each other.
% As the highest disparity is reported due to speech rate and discline group feature, we observed the disparity exists in ASR performance (H=223.2,$p\leq 0.001$) at the intersection of these two features too.

% \begin{table}[!t]
% \centering
% \begin{tabular}{lccc}
% \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Discipline Group}}} & \multicolumn{3}{c}{\textbf{Speech Rate}} \\ \cline{2-4} 
% \multicolumn{1}{l|}{} & \multicolumn{1}{l}{Slow} & \multicolumn{1}{l}{Average} & \multicolumn{1}{l}{Fast} \\ \hline
% Non-Engineering & 14.4 & 12.6 & 13.0 \\
% Engineering & 15.7 & 14.8 & 14.2 \\ \hline
% \end{tabular}
% \caption{Median WER (\%)  of speakers for YouTube ASR \sjnote{fix caption}}
% \label{tab:disc_speech_yt}

% \end{table}

\begin{table}[!t]
    \centering
    \small
    \begin{tabular}{|c|c|c|c|}
        \hline
        \multirow{2}{*}{\textbf{Discipline}} & \multicolumn{3}{c|}{\textbf{Speech Rate}} \\
        \cline{2-4}
         & \textbf{Slow} & \textbf{Avg.} & \textbf{Fast} \\
         \hline
         Non-Engineering & 14.4 & 12.6 & 13.0 \\
         \hline
         Engineering & 15.7 & 14.8 & 14.2 \\ 
         \hline
    \end{tabular}
    \caption{Median WER (\%)  of speakers for YouTube ASR \todo{fix caption}}
    \label{tab:yt_disc_speech}
\end{table}

\subsubsection{ Intersectional Disparity}
We have evaluated the performance of the YouTube ASR for intersectional categories by combining speech rate and discipline. From Table~\ref{tab:yt_disc_speech}, we see that there is a statistically significant ($H$ = 223.2, $p\leq$ 0.001) disparity between the intersectional categories. Next, from Figure~\ref{fig:yt_speech_discipline}, we see that the highest WER (15.7\%) is reported for slow speakers in the engineering discipline whereas the lowest WER (12.6\%) is reported for fast speakers in non-engineering discipline. Correspondingly, these two categories have the highest (10.7\%) and lowest (XX) IQR as well.

\noindent \paragraph{Takeaways:} We now state the takeaways from the intersectional experiments--
% From Figure \ref{fig:speech_discipline_yt} and Table \ref{tab:disc_speech_yt}, it has been observed that:
\begin{itemize}
   \item  The YouTube ASR has the worst performance for engineering lecture videos where the speakers have a slow speech rate.
   % YouTube ASR performs worst on engineering lectures delivered with slow speech rate having WER median of 15.7\% and IQR of 10.7\% .
   \item The lowest WER (12.6\%) is reported for non-engineering lecture videos delivered with an average speech rate. This is 3.1\% less than the above mentioned group.
   % For non-engineering lectures delivered with average speech rate, the WER median is lowest at 12.6\% having disparity with 3.1\% with above-mentioned group.
   \item From Figure~\ref{fig:yt_speech_discipline}, highest disparity of 4\% in IQR between slow-engineering group and fast non-engineering subgroups is observed. \sjnote{If lowest is for avg speed+non-engg, how is disparity highest between these two? }
   \item From Fig.~\ref{fig:yt_speech_discipline}, we see that the box plots for the non-engineering category have consistently lower dispersion compared to their counterparts for the engineering category.
   % Figure \ref{fig:speech_discipline_yt} shows boxplots corresponding non-engineering category has consistently low dispersion from their corresponding counterparts in engineering domain.
\end{itemize}

\if{0}
\ref{fig_5} shows highest WER median of 15.7\% and IQR of 10.7\%  for engineering lectures delivered with slow speech rate while lowest WER median of 12.9\% and IQR of 6.9\%  for non-engineering lectures delivered with fast speech rate.
\fi

\begin{figure*}[ht]
	\centering
	\begin{subfigure}{0.75\columnwidth}
		\includegraphics[width= \textwidth, height=8cm, keepaspectratio]{figures/speech_discipline_yt.pdf}
		\caption{YouTube}
		\label{fig:yt_speech_discipline}
	\end{subfigure}
	~\begin{subfigure}{0.75\columnwidth}
		\includegraphics[width= \textwidth,  height=8cm, keepaspectratio]{figures/speech_discipline_wp.pdf}
		\caption{Whisper}
		\label{fig:wsp_speech_discipline}
	\end{subfigure}%
       \caption{WER Disparity on Intersection of Speech Category and Discipline Group in YouTube and Whisper ASR \sjnote{Use patterns like -- 'x', 'o', '.' instead of colours. We haven't used colours elsewhere and we should be uniform.}}
       \label{fig:speech_discipline_comp}
 \end{figure*}
	
	
\subsection{Whisper}
In the ASR Comparison subsection , we have reported that the Whisper model outperformed the YouTube Automatic Captions on TIE dataset and there is a strong correlation between WER distribution of both ASR models. Now, having analyzed the effect of different features on YouTube ASR model, we would like to see the impact of same features on the Whisper model.  

It is also to be noted that in the ~\cite{radford2022robust} paper, OpenAI has benchmarked its Large V2 model on many publicly available datasets ~\cite{CORAAL,meyer2020artie} but they have not reported the performance based on demographic aspects of the speakers present in the dataset which makes our below findings very relevant.

\begin{table}[!t]
    \small
    \centering
    \begin{tabular}{|c|c|c|l|}
    \hline
     \textbf{Category} & \textbf{Attribute} & \textbf{WER (\%)} & \textbf{Test}\sjnote{what test?}\\
     \hline
     \multirow{2}{*}{\textbf{Gender}} & Female & 9.6 & \multirow{2}{*}{$H$ = 87.1, $p$ \textless 0.001} \\
     \cline{2-3}
     & Male & \textbf{11.9} & \\ 
     \hline\hline
     \multirow{2}{*}{\textbf{Caste}} & RES & 11.4 & \multirow{2}{*}{$H$ = 6.4, $p$ \textgreater 0.001} \\
     \cline{2-3}
     & UR & \textbf{11.9} & \\ 
     \hline\hline
     \multirow{4}{*}{\textbf{Exp.}} & $\leq$ 1980 & \textbf{13.3} & \multirow{4}{*}{$H$ = 135.8, $p$ \textless 0.001} \\
     \cline{2-3}
     & 1981-90 & 11.5 & \\ 
     \cline{2-3}
     & 1991-00 & 11.9 & \\ 
     \cline{2-3}
     & $\geq$ 2001 & 11.2 & \\ 
     \hline\hline
     \multirow{4}{*}{\textbf{Native}} & North & 10.8 & \multirow{4}{*}{$H$ = 80.3, $p$ \textless 0.001} \\
     \cline{2-3}
     & South & \textbf{12.4} & \\ 
     \cline{2-3}
     & East & 11.6 & \\ 
     \cline{2-3}
     & West & 11.4 & \\ 
     \hline\hline
     \multirow{3}{*}{\textbf{Speech Rate}} & Slow & \textbf{9.3} & \multirow{3}{*}{$H$ = 160.6, $p$ \textless 0.001} \\
     \cline{2-3}
     & Avg. & 7.8 & \\ 
     \cline{2-3}
     & Fast & 7.4 & \\ 
     \hline\hline
    \multirow{2}{*}{\textbf{Discipline}} & Non-Eng. & 11.0 & \multirow{2}{*}{$H$ = 128.9, $p$ \textless 0.001} \\
     \cline{2-3}
     & Engg. & \textbf{12.2} & \\ 
     \hline
    \end{tabular}
    \caption{Word Error Rate (WER) and XX Test\sjnote{what test?} results for transcripts generated by OpenAI Whisper ASR. \sjnote{should we combine YTB and WSPR in a single table?}}
    \label{tab:wsp_comparison_tbl}
\end{table}

% \begin{table}[ht]
% \caption{Results on Whisper}
% \label{tab:whisper_compar_tbl}
% \begin{tabular}{cccl}
% \hline
% \multicolumn{1}{l}{\textbf{Category}} & \multicolumn{1}{l}{\textbf{Attribute}} & \multicolumn{1}{l}{\textbf{WER (\%)}} & \multicolumn{1}{c}{\textbf{Test Result}} \\ \hline
% \multirow{2}{*}{\textbf{Gender}} & Female & 9.6 & \multicolumn{1}{c}{\multirow{2}{*}{H=87.1,p\textless{}0.001}} \\
%  & Male & 11.9 & \multicolumn{1}{c}{} \\ \hline
% \multirow{2}{*}{\textbf{Caste}} & RES & 11.4 & \multicolumn{1}{c}{\multirow{2}{*}{H=6.4, p\textgreater{}0.001}} \\
%  & UR & 11.9 & \multicolumn{1}{c}{} \\ \hline
% \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Teaching \\ Since\end{tabular}}} & \textless{}=1980 & 13.3 & \multicolumn{1}{c}{\multirow{4}{*}{H=135.8,p\textless{}0.001}} \\
%  & 1981-90 & 11.5 & \multicolumn{1}{c}{} \\
%  & 1991-00 & 11.9 & \multicolumn{1}{c}{} \\
%  & \textgreater{}=2001 & 11.2 & \multicolumn{1}{c}{} \\ \hline
% \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Native\\ Region\end{tabular}}} & East & 11.6 & \multirow{4}{*}{H=80.3,p\textless{}0.001} \\
%  & West & 11.4 &  \\
%  & North & 10.8 &  \\
%  & South & 12.4 &  \\ \hline
% \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Speech \\ Rate\end{tabular}}} & Slow & 9.3 & \multirow{3}{*}{H=160.6,p\textless{}0.001} \\
%  & Average & 7.8 &  \\
%  & Fast & 7.4 &  \\ \hline
% \multicolumn{1}{l}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Discipline\\ Group\end{tabular}}}} & Non-Eng. & 11.0 & \multirow{2}{*}{H=128.9,p\textless{}0.001} \\
% \multicolumn{1}{l}{} & Eng. & 12.2 &  \\ \hline
% \end{tabular}
% \end{table}


\begin{figure*}[t]
    \centering
	~\begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/gender_wp.pdf}
		\caption{Gender}
		\label{fig:wsp_gender}
	\end{subfigure}%
	~\begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/caste_wp.pdf}
		\caption{Caste}
		\label{fig:wsp_caste}
	\end{subfigure}%
	~\begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/age_wp.pdf}
		\caption{Experience}
		\label{fig:wsp_exp}
	\end{subfigure} 
    \begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/region_wp.pdf}
		\caption{Native Region}
		\label{fig:wsp_native}
	\end{subfigure}
	~\begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/speech_wp.pdf}
		\caption{Speech Rate}
		\label{fig:wsp_speed}
	\end{subfigure}
	~\begin{subfigure}{0.32\columnwidth}
		\includegraphics[width= \textwidth, height=3cm, keepaspectratio]{figures/discipline_wp.pdf}
		\caption{Discipline}
		\label{fig:wsp_discipline}
	\end{subfigure}
	\caption{WER Disparity across various attributes for OpenAI Whisper ASR.}
	\label{fig:wsp_word_error_rate}
\end{figure*}

% \begin{figure*}[ht]
	
% 	\begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=4cm, keepaspectratio]{figures/gender_wp.pdf}
% 		\caption{Gender}
% 		\label{fig:wp_word_error_rate_a}
% 	\end{subfigure} \hfill%
% 	~\begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=4cm, keepaspectratio]{figures/caste_wp.pdf}
% 		\caption{Caste Category}
% 		\label{fig:wp_word_error_rate_b}
% 	\end{subfigure}%
% 	~\begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=4cm, keepaspectratio]{figures/age_wp.pdf}
% 		\caption{Exp. Category}
% 		\label{fig:wp_word_error_rate_c}
% 	\end{subfigure}%
 
%  \begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=4cm, keepaspectratio]{figures/region_wp.pdf}
% 		\caption{Native Region}
% 		\label{fig:wp_word_error_rate_d}
% 	\end{subfigure}\hfill% \hspace{2}
% 	~\begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=4cm, keepaspectratio]{figures/speech_wp.pdf}
% 		\caption{Speech Rate Category}
% 		\label{fig:wp_word_error_rate_e}
% 	\end{subfigure}
% 	~\begin{subfigure}{0.66\columnwidth}
% 		\includegraphics[width= \textwidth, height=4cm, keepaspectratio]{figures/discipline_wp.pdf}
% 		\caption{Discipline Category}
% 		\label{fig:wp_word_error_rate_f}
% 	\end{subfigure}
% 	\caption{WER Disparity across various attributes for OpenAI Whisper Model }
% 	\label{fig:yt_word_error_rate}
% \end{figure*}

\subsubsection{Gender Disparity}
Even with the better overall performance on the TIE dataset, it is surprising there is a significant difference (H=87.1,$p\leq 0.001$) in the model performance due to perceived gender attribute of the speaker.
\noindent \paragraph{Takeaways:}  From Figure \ref{fig:wp_word_error_rate_a} and Table \ref{tab:whisper_compar_tbl}, it has been observed that:
\begin{itemize}
   \item Whisper Model favors female voices compared to male voices with a significant median difference of 2.3\%.
   \item From Figure \ref{fig:wp_word_error_rate_a} , it can be observed the IQR dispersion for female speakers is less spread than that of males.
   
\end{itemize}


\subsubsection{Caste Disparity}

\noindent \paragraph{Takeaways:}  From Figure \ref{fig:wp_word_error_rate_b} and Table \ref{tab:whisper_compar_tbl}, it has been concluded  that:

\begin{itemize}
    \item No significant disparity  is found in performance of Whisper Model due to caste factor of speaker
\end{itemize}
 

\subsubsection{Age Group Disparity}

Whisper model exhibits significant model performance disparity due to speaker's age factor.

\noindent \paragraph{Takeaways:}  From Figure \ref{fig:wp_word_error_rate_c} and Table \ref{tab:whisper_compar_tbl}, it has been concluded  that:

\begin{itemize}
    \item The highest disparity in  WER median for Whisper Model generated transcripts of  2.0\% is seen between for speakers of highest experience category and lowest experienced category speakers.
    \item The IQR dispersion reduces from 9.8\% to 7.4\% as we move from instructors teaching before 1980 to instructors started teaching after 2001.
\end{itemize}




\subsubsection{Native Region Disparity}
The difference in English accents of speakers from North and South Indian regions may be attributed to the disparity in performance of Whisper model. 

\noindent \paragraph{Takeaways:}  From Figure \ref{fig:wp_word_error_rate_d} and Table \ref{tab:whisper_compar_tbl}, it has been concluded  that:

\begin{itemize}
    \item The model performs best for North Indian English accent, followed by speakers native from Western ,Eastern and Southern  parts of India.
    \item The variation of IQR dispersion is highest for East and West Indian speakers as per \ref{fig:wp_word_error_rate_d}. 
\end{itemize}


\subsubsection{Speech Rate Disparity }
The disparity in performance is observed due to speech rate of the audio file being transcribed.

\noindent \paragraph{Takeaways:}  From Figure \ref{fig:wp_word_error_rate_e} and Table \ref{tab:whisper_compar_tbl}, it has been concluded  that:

\begin{itemize}
    \item The lecture with fast speech rate is accurately transcribed by Whisper  than the lecture with slow speech rate and the difference of median WER between two is 1.5\%.
    \item  Whisper model transcription performance consistency is inversely proportional to speech rate category with IQR for Fast, Average and Slow speed  as per \ref{fig:wp_word_error_rate_e}. 
\end{itemize}

\subsubsection{Discipline Group Disparity}
Even with 680,000 hours of multilingual and multitask supervised training ~\cite{radford2022robust}, the resulting Whisper model does not generalize well for engineering group disciplines when compared with non-engineering group disciplines(H=128.9,$p\leq 0.001$).

\noindent \paragraph{Takeaways:}  From Figure \ref{fig:wp_word_error_rate_f} and Table \ref{tab:whisper_compar_tbl}, it has been concluded  that:

\begin{itemize}
    \item There is significant difference of 1.2\% in WER median for engineering and non-engineering discipline groups is  is 
    \item  The IQR difference between both groups is 1.9\% depicting consistently better  transcription of lectures related to Non-Engineering disciplines as per \ref{fig:wp_word_error_rate_f}. 
\end{itemize}



\subsubsection{Intersection Disparity}

The highest disparity(H=320.5,$p\leq 0.001$) is observed at intersection of Speech rate and Discipline Group attribute.

\noindent \paragraph{Takeaways:}  From Figure \ref{fig:speech_discipline_wp}, it has been concluded  that:

\begin{itemize}
    \item The highest WER median of 13.2\% and IQR of 10.4\%  for engineering lectures delivered with slow speech rate while lowest WER median of 11.0\% and IQR of 6.9\%  for non-engineering lectures delivered with fast speech rate. 
\end{itemize}

. 
